Tackling the Non-IID Issue in Heterogeneous Federated Learning by Gradient Harmonization

Federated learning (FL) is a privacy-preserving paradigm for collaboratively training a global model from decentralized clients. However, the performance of FL is hindered by non-independent and identically distributed (non-IID) data and device heterogeneity. In this work, we revisit this key challenge through the lens of gradient conflicts on the server side. Specifically, we first investigate the gradient conflict phenomenon among multiple clients and reveal that stronger heterogeneity leads to more severe gradient conflicts. To tackle this issue, we propose FedGH, a simple yet effective method that mitigates local drifts through Gradient Harmonization. This technique projects one gradient vector onto the orthogonal plane of the other within conflicting client pairs. Extensive experiments demonstrate that FedGH consistently enhances multiple state-of-the-art FL baselines across diverse benchmarks and non-IID scenarios. Notably, FedGH yields more significant improvements in scenarios with stronger heterogeneity. As a plug-and-play module, FedGH can be seamlessly integrated into any FL framework without requiring hyperparameter tuning.

==> sections/2_related.tex <==
\section{Related Works}
\subsection{Federated Learning}
\cite{FedAvg} propose a solid baseline in FL termed FedAvg, 
which directly averages local models to update the global model. 
However, \cite{scaffold} identify that FedAvg yields unstable and slow convergence in heterogeneous scenarios, 
and \cite{FedProx} further subdivide the non-IID issue into systems heterogeneity and statistical heterogeneity. 
To tackle this key challenge, researchers have elaborated different strategies from different steps of FL. 

During local training, many promising methods focus on regularizing the local objective. 
Specifically, \cite{FedProx} introduce a proximal term to minimize the gap between local and global models, 
while \cite{FedDyn} align these models via dynamic regularization. 
Additionally, \cite{MOON} employ model-level contrastive learning to correct local updates, 
and \cite{FedDECORR} tackle the non-IID issue from the dimensional collapse perspective. 
Moreover, the pursuit of flatter local minima is explored in \cite{FedSAM} and \cite{FedSAM2} by applying a sharpness-aware optimizer.

On the server side, aggregation of local models and updating of the global model are two directions for addressing the non-IID problem. 
\cite{FedNova} propose a normalized averaging scheme instead of the naïve aggregation in FedAvg. 
In addition, \cite{FedMA} and \cite{FedLA} aggregate local models in a layer-wise manner, while \cite{Outlier} introduce an outlier pruning strategy before aggregation. 
On the other hand, \cite{FedAvgM}, \cite{Slowmo}, and \cite{FedOpt} demonstrate that incorporating momentum-based updates into the global model is beneficial for mitigating local drift. 
However, our proposed FedGH is orthogonal to these methods and can be easily embedded in other FL frameworks.

\subsection{Gradient Surgery}
\cite{PCGrad} first identify that conflicting gradients lead to performance degradation in multi-task learning, 
introducing PCGrad to enhance optimization performance via gradient surgery. 
Subsequently, \cite{DGGS} extend this insight to domain generation, presenting two gradient agreement strategies to alleviate gradient conflict. 
Moreover, DOHA introduce a sample-wise gradient deconfliction technique to boost generalization performance. In contrast, we uncover the gradient conflict phenomenon in FL caused by the non-IID issue. 
Our work centers on client-wise gradient harmonization during server aggregation rather than gradient surgery in every training iteration \cite{PCGrad, DGGS}. Thus, FedGH is computationally efficient without introducing any extra communication costs.

\label{sec:related}
